Balancing Specialization, Generalization, and Compression for Detection and Tracking

We propose a method for specializing deep detectors and trackers to restricted settings. Our approach is designed with the following goals in mind: (a) Improving accuracy in restricted domains; (b) preventing overfitting to new domains and forgetting of generalized capabilities; (c) aggressive model compression and acceleration. To this end, we propose a novel loss that balances compression and acceleration of a deep learning model vs. loss of generalization capabilities. We apply our method to the existing tracker and detector models. We report detection results on the VIRAT and CAVIAR data sets. These results show our method to offer unprecedented compression rates along with improved detection. We apply our loss for tracker compression at test time, as it processes each video. Our tests on the OTB2015 benchmark show that applying compression during test time actually improves tracking performance.

==> our_bmvc_reviews.tex <==
Questions
1. [ Paper Summary ] What is this paper about? Please be concise (3-5 sentences) Type: Comment
This paper presents a visual tracker that solves the balance problem of generalization and adaptation. The detection performance is evaluated using VIRAT and CAVIAR datasets, while the visual tracking performance is evaluated using the OTB2015 dataset.
2. [ Paper Strengths ] Please summarize the strengths of the paper. (Eg: novelty, insight, theoretical strength, state of the art performance, thorough evaluation)
The method attempts to define visual tracking problems into two categories. One is Model specialization vs. generalization and the other is model compression vs. acceleration. This definition is well motivated and the problems related to them are very important in visual tracking. 

The above mentioned issues are well addressed using simple losses in the paper. The numerical results demonstrate the effectiveness of the proposed techniques. 
These techniques can be easily integrated into conventional visual trackers. 

3. [ Paper Weaknesses ] Please summarize the weaknesses of the paper. (E.g., Lack of novelty, technical errors, insufficient evaluation, etc). You should justify your criticisms (E.g., with an explanation of technical errors, citation to prior work if novelty is an issue). It is not appropriate to ask for comparison with unpublished arXiv papers, and papers published after the BMVC deadline. Please be polite and constructive.
The drawback of this paper is insufficient experiments on visual tracking. The performance of the proposed visual tracker needs to be evaluated using VOT, UAV123, LaSOT, and TC-128 datasets.
4. [ Detailed Comments ] Any further detailed comments to the authors, including suggestions for improving the camera ready version, if accepted.
The further evaluations using additional visual tracking datasets will make the method stronger.
5. [ Overall Rating ]
Accept
Reviewer #2
Questions
1. [ Paper Summary ] What is this paper about? Please be concise (3-5 sentences) Type: Comment
This paper presents a method to compress deep models for detection and tracking. Specifically, the authors propose a loss to balance compression and acceleration of a deep learning model vs. loss of generalization capabilities.
2. [ Paper Strengths ] Please summarize the strengths of the paper. (Eg: novelty, insight, theoretical strength, state of the art performance, thorough evaluation)
This paper is clearly written. The main pipeline of the proposed algorithm is easy to follow. Experimental results show the effectiveness of the proposed method to some extent on the detection benchmarks.
3. [ Paper Weaknesses ] Please summarize the weaknesses of the paper. (E.g., Lack of novelty, technical errors, insufficient evaluation, etc). You should justify your criticisms (E.g., with an explanation of technical errors, citation to prior work if novelty is an issue). It is not appropriate to ask for comparison with unpublished arXiv papers, and papers published after the BMVC deadline. Please be polite and constructive.
The novelty of this paper is not significant. The authors simply combine two losses with a hyperparameter. While it is interesting in its own right, the contributions seem to be marginal. 

This paper is not presented well. The authors do not provide baseline detection and tracking methods for a fair comparison. It is difficult for readers to understand how the performance of the compressed models for detection and tracking. Both Fig. 2 and Fig. 3 are not clear enough to understand the performance of the detector and tracker.
4. [ Detailed Comments ] Any further detailed comments to the authors, including suggestions for improving the camera ready version, if accepted.
The reviewer leans towards recommending an acceptance if the authors provide more insights into the proposed loss, e.g., why a straightforward combination works well, and add more baseline detectors and trackers for comparison.
5. [ Overall Rating ]
Borderline Accept
Reviewer #3
Questions
1. [ Paper Summary ] What is this paper about? Please be concise (3-5 sentences) Type: Comment
This paper focused on improving the performance of deep models on restricted settings, such as low delay scenarios. For this aim, the authors proposed a loss function that considers compression and network runtime of a deep learning model. The results showed that applying compression during test time improves tracking performance.
2. [ Paper Strengths ] Please summarize the strengths of the paper. (Eg: novelty, insight, theoretical strength, state of the art performance, thorough evaluation)
The paper address a problem of computation and storage in deep learning models. The paper is well-written until the beginning of the most important part - 3.3 Compression and acceleration. I would say only novelty is the combination of the forgetting and compute cost in lost function.
3. [ Paper Weaknesses ] Please summarize the weaknesses of the paper. (E.g., Lack of novelty, technical errors, insufficient evaluation, etc). You should justify your criticisms (E.g., with an explanation of technical errors, citation to prior work if novelty is an issue). It is not appropriate to ask for comparison with unpublished arXiv papers, and papers published after the BMVC deadline. Please be polite and constructive.
As the paper focuses on improving compression and network runtime, experimental evaluation and results are needed to formulate more clearly to show how much the network runtime improved after the proposed model. The current version of the paper does not clearly describe the idea of compression of the model. It seems that the authors did not spend much time on the last part of the paper (e.g., 4.4 and result sections). Also, it is not clear how the authors measure the network runtime.
4. [ Detailed Comments ] Any further detailed comments to the authors, including suggestions for improving the camera ready version, if accepted.
I suggest the authors improve the result part of the paper, and include the network runtime results and provide runtime comparison with reference methods.
5. [ Overall Rating ]
Borderline Reject



META-REVIEW QUESTIONS
1. 1. [ Meta Review ] Please enter your meta-review here. Your report should address the key points brought up by the reviewers, and summarise any ensuing discussion. You should provide enough information that the authors understand the reasons for the recommendation. Particularly if there are split reviews, explain how you made your decision. E.g., "R1's point that the method is novel out-weighted R2's concern that the evaluation could have been more thorough". or "R3's flagging a theoretical error out-weighed R1's support for state of the art results". Obviously your comments should agree your overall accept/reject recommendation below.
The reviews for this paper are A, BA and BR. Reviewers raise questions about the experiments and the method itself, but the work clearly proposes ideas that will widely interest conference audience and thus deserves to be published.
META-REVIEWER #2
META-REVIEW QUESTIONS
1. 1. [ Meta Review ] Please enter your meta-review here. Your report should address the key points brought up by the reviewers, and summarise any ensuing discussion. You should provide enough information that the authors understand the reasons for the recommendation. Particularly if there are split reviews, explain how you made your decision. E.g., "R1's point that the method is novel out-weighted R2's concern that the evaluation could have been more thorough". or "R3's flagging a theoretical error out-weighed R1's support for state of the art results". Obviously your comments should agree your overall accept/reject recommendation below.
Two reviewers recommend acceptance, while R3 rates the paper as Borderline Reject. All reviewers express some concerns about the experimental evaluation, particularly regarding compression. While the paper will be of interest to the community, we strongly encourage the authors to take the reviewers' comments into account for the final version.

